Inference on Auctions with Weak Assumptions on Information

Given a sample of bids from independent auctions, this paper examines the question of inference on auction fundamentals (e.g. valuation distributions, welfare measures) under weak assumptions on information structure. The question is important as it allows us to learn about the valuation distribution in a robust way, i.e., without assuming that a particular information structure holds across observations. We leverage the recent contributions of \cite{Bergemann2013} in the robust mechanism design literature that exploit the link between Bayesian Correlated Equilibria and Bayesian Nash Equilibria in incomplete information games to construct an econometrics framework for learning about auction fundamentals using observed data on bids. We showcase our construction of identified sets in private value and common value auctions. Our approach for constructing these sets inherits the computational simplicity of solving for correlated equilibria: checking whether a particular valuation distribution belongs to the identified set is as simple as determining whether a {\it linear} program is feasible. A similar linear program can be used to construct the identified set on various welfare measures and counterfactual objects. For inference and to summarize statistical uncertainty, we propose novel finite sample methods using tail inequalities that are used to construct confidence regions on sets. We also highlight methods based on Bayesian bootstrap and subsampling. A set of Monte Carlo experiments show adequate finite sample properties of our inference procedures. We illustrate our methods using data from OCS auctions.

==> counterfactual.tex <==
 Suppose that we wanted to understand the performance of some other auction when deployed in the same market, with respect to some metric: $W:V^n\times B\rightarrow \R$ that is a function of the unknown value vector and the bid vector in the private value setting or a function $W:V\times B\rightarrow \R$ in the common value setting. Examples of such metrics could be social welfare: $W(v,b)=\sum_{i=1}^n v_i x_i(b)$  or revenue, i.e. $W(v,b)=\sum_{i=1}^n \Theta_I(b)$, where $x_i(b)$ is the probability of allocating to player $i$ under bid profile $b$ and $\Theta_I(b)$ is the expected payment of player $i$ under bid profile $b$.

 We are interested in computing an upper and lower bound on this metric under this new auction which has different utilities $\tilde{u}_i(b;\theta)$ and under any Bayes-correlated equilibrium. This is important since it allows us to obtain bounds on welfare or other metrics in a new environment under general information structures. The welfare bounds computed in this manner will inherit the robustness property in that they will be valid under all information structures. 

This is straightforward in our setup since computing a sharp identified set for any such counter-factual can be done in a computationally efficient manner, in both the common value setting and in the correlated private value setting. The upper bound of the counter-factual boils down to the following linear program (we give here the linear program for the case of common values, but the analogous program can be written for correlated private values), that takes as input the observed distribution of bids in our current auction, the metric $W$ and the primitive utility form $\tilde{u}=(\tilde{u}_1,\ldots,\tilde{u}_n)$ under the alternative auction. We state this in the next Theorem.

\begin{theorem}
	Let the common value model above hold. Given a social welfare function $W:V\times B\rightarrow \R$, $\phi(),$ and vector of utilities $\tilde u$, the sharp upper and lower bounds on expected welfare can be computed using the following LP:
 \begin{align*}
 LP(\phi,W,\tilde{u}) ~~~&~~~ \underset{\tilde{\psi}}{\min/\max}\sum_{v,b} W(v,b) \cdot \tilde{\psi}(v,b)  \\ 
 ~~~&~~~ \forall b_i,b_i':  \sum_{v\in V, b_{-i}\in B^{n-1}} \tilde{\psi}(v,b)\cdot \left(\tilde{u}_i(b;v)-\tilde{u}_i(b_i',b_{-i};v)\right) \geq 0\\
 ~~~&~~~ \forall v\in V:~  \pi(v) = \sum_{b\in B^{n}} \tilde{\psi}(v,b)\\
 ~~~&~~~  \tilde{\psi} \in \Delta(V\times B^n) \text{ and } \pi \in \Pi_I(\phi)
 \end{align*}
 \end{theorem}
 Similarly if we want to compute a lower bound on the counter-factual we can compute the minimum rather than the maximum of the above objective subject to the same constraints.
